Attribute-Based Encryption for Circuits from Multilinear Maps

In this work, we provide the first construction of Attribute-Based Encryption (ABE) for general circuits. Our construction is based on the existence of multilinear maps. We prove selective security of our scheme in the standard model under the natural multilinear generalization of the BDDH assumption. Our scheme achieves both Key-Policy and Ciphertext-Policy variants of ABE.

==> lattice.tex <==
\section{Conversion to the GGH multilinear framework}

The circuit-ABE scheme we outline above can be adapted to the Garg-Gentry-Halevi framework in a fairly straightforward manner,
and the security will hold under a multi-DDH-style assumption, such as the one formulated by GGH.

The main obstacle to directly using the GGH framework is the domain where the ``exponents'' in our scheme and proof
come from.  In the GGH framework, this domain must essentially be ``small'' polynomials (we will think of them as corresponding
to a unique representative modulo the $g$ polynomial that defines the ideal $I$ in the GGH framework).

We will use different bounds of ``smallness'' at each level.  More precisely, let us assume that our measure of shortness $||\cdot||$
satisfies the following constraint:

For fixed degree polynomials $c_1, c_2, \dots c_m$ such that $||c_i|| < 2^k$,
we have that 
$$||c_1 \cdots c_m|| < f(m) 2^{km} $$
for some quasi-singly-exponential, strictly increasing, function $f$.
This constraint is satisfied by all standard measures of the size of a polynomial over $\mathbb{Z}$.

Then, at level $i$, i.e. in $G_i$ above, when picking a random element, we will choose
an element of size $f(i+1)2^{(i+1)k}$.

The only exception will be $s$, which we will choose of size $2^k$.  

Finally, in the multi-DDH-style assumption, we will require security to hold when $s$ and all the $a_i$
are each chosen from size $2^k$.

\paragraph{Impact on proof of security.}
By choosing our randomness in this way, the main fact we will rely on is that
if $a$ is chosen randomly of size $A$, and $b$ is chosen randomly of size $B$,
where $A > B 2^k$, then the distribution $a+b$ is exponentially close to the distribution $a$.

This will allow the proof of security to go through with only exponentially small statistical loss due to 
the distribution being slightly different in the proof of security vs. the real-life game.


 
